Online Discrepancy Minimization for Stochastic Arrivals

In the stochastic online vector balancing problem, vectors $v_1,v_2,\ldots,v_T$ chosen independently from an arbitrary distribution in $\mathbb{R}^n$ arrive one-by-one and must be immediately given a $\pm$ sign. The goal is to keep the norm of the discrepancy vector, i.e., the signed prefix-sum, as small as possible for a given target norm. We consider some of the most well-known problems in discrepancy theory in the above online stochastic setting, and give algorithms that match the known offline bounds up to $\mathsf{polylog}(nT)$ factors. This substantially generalizes and improves upon the previous results of Bansal, Jiang, Singla, and Sinha (STOC' 20). In particular, for the Koml\'{o}s problem where $\|v_t\|_2\leq 1$ for each $t$, our algorithm achieves $\tilde{O}(1)$ discrepancy with high probability, improving upon the previous $\tilde{O}(n^{3/2})$ bound. For Tusn\'{a}dy's problem of minimizing the discrepancy of axis-aligned boxes, we obtain an $O(\log^{d+4} T)$ bound for arbitrary distribution over points. Previous techniques only worked for product distributions and gave a weaker $O(\log^{2d+1} T)$ bound. We also consider the Banaszczyk setting, where given a symmetric convex body $K$ with Gaussian measure at least $1/2$, our algorithm achieves $\tilde{O}(1)$ discrepancy with respect to the norm given by $K$ for input distributions with sub-exponential tails. Our key idea is to introduce a potential that also enforces constraints on how the discrepancy vector evolves, allowing us to maintain certain anti-concentration properties. For the Banaszczyk setting, we further enhance this potential by combining it with ideas from generic chaining. Finally, we also extend these results to the setting of online multi-color discrepancy.

==> banasczyck.tex <==
\newcommand{\diam}{\mathsf{diam}}

\newpage

\section{Discrepancy for Arbitrary Convex Bodies}

In this section, we prove the following  theorem which uses a stronger potential than used in the previous section. Later in Section \ref{sec:banasczyck} and Section \ref{sec:subgaussian} we will use this to bound the discrepancy in any arbitrary norm as well as combine it with the min-max theorem to imply the existence of an online algorithm that produces a $\polylog(T)$-subgaussian distribution over discrepancy vectors. \\

To state the result, we use the same notation as in the previous section. Let $V \in \BR^n$ be our input random vector with $\|V\|_2 \le 1$ and $\tM_k$ be as stated in \eqref{eqn:matdecomp}. 

\mnote{For now this statement is only for a single scale.}

\begin{theorem}\label{thm:gen-disc-ban}
    Let $r > 0$ and $\CZ \subseteq \BR^n$, $|\CZ|\le 2^{r^2}$ be a set of test vectors of Euclidean length $r$. Then, for vectors $v_1, \ldots, v_T$ sampled i.i.d. from $\sfp(V)$, there is an online algorithm that w.h.p. maintains the following for the discrepancy  vector $d_t$ at any time $t$,
    \[ \max_{z \in \CZ} |d_t^T z| \le r^2 \log T.\] 
\end{theorem}

\subsection{Discrepancy for an arbitrary norm}

\subsection{Proof of Theorem \ref{thm:gen-disc-ban}}


\paragraph{New Potential Function and Algorithm.}

Recall the notation used in \eqref{eqn:eigendecomp} and \eqref{eqn:matdecomp}. As before, to define the potential, we first define a distribution which is a noisy version of the input distribution where some noise is added to account for the test directions. Let $W \in \BR^n$ be an independent copy of $V$ and $Z$ be uniform over $\CZ$. Let $X \in \BR^n$ equal $W$ or $Z$ with probability $1/2$ each. As before, $\|X\|_2 \le 1$ since $\|M\|_{\op} \le 1$.\\

At any time step $t$, let $d_{t} = \chi_1 v_1 + \ldots + \chi_t v_t$ denote the current discrepancy vector after the signs $\chi_1, \ldots, \chi_t \in \{\pm1\}$ have been chosen. Set $\lambda^{-1} = 12\log^2(nT)$ and define the potential 
\[ \Phi_t = \Phi(d_t) := \sum_{k=0}^{\kappa} \BE_{p(x)}\left[\exp\left(\lambda^2 (d_{t}^T \tM_k x)^2\right)\right]. \]

When the vector $v_t$ arrives, the algorithm chooses the sign $\chi_t$ that minimizes the increase $\Phi_t - \Phi_{t-1}$.\\

\paragraph{Analysis.} The analysis of this algorithm is quite similar to the analysis we encountered in Komlos's setting. In particular, we have the following lemma analogous to Lemma \ref{lemma:tail}. Let $\CG_t = \CG(d_t)$ denote the set of vectors in the support of $\sfp(V)$ such that $\lambda^2|d_t^T \tM_k v|^2 \le \log (2 \Phi_t/\delta)$ for every $k \le \kappa$. 

\begin{lemma}\label{lemma:gen-tail}
For any $\delta > 0$, the following holds at any time $t$, $\sfp(V \notin \CG_t) \le \delta$.
\end{lemma}
\begin{proof}
 As defined above, we have that $X=W$ with probability $1/2$ where $W$ is an independent copy of $V$. Therefore,   $\BE_{w}\left[\exp(\lambda^2 |d_t^T\tM_k w|^2)\right] \le 2 \Phi_t$ for any $k \le \kappa$. By an application of Markov's inequality, it follows that $\sfp(V \notin \CG_t) = \sfp(W \notin \CG_t) \le \delta$.\mnote{Readjust parameters to account for a union bound.}
\end{proof}

\vspace*{8pt}
The next lemma shows that the expected increase (or drift) in the potential is small on average.
\begin{lemma}[Drift]\label{lemma:gen-drift} At any time $t$ if $T \le \Phi_{t-1} \le T^4$, then $\BE_{v_t}[\Phi_t] - \Phi_{t-1} \le 2.$
\end{lemma}

Lemma \ref{lemma:gen-drift} implies that for any time $t \in [T]$, the expected value of the potential $\Phi_t$ over the input sequence $v_1, \ldots, v_T$ is at most $3T$. By Markov's inequality, it follows that with probability at least $1-T^{-4}$, the potential $\Phi_t \le 3T^5$ for every $t \in [T]$. This proves Theorem \ref{thm:gen-disc}. To finish the proof we prove Lemma \ref{lemma:gen-test} next.

\begin{proof}[Proof of Lemma \ref{lemma:gen-drift}]

Let us fix a time $t$. To simplify the notation, let $\Phi = \Phi_{t-1}$ and $\Delta\Phi = \Phi_t - \Phi$, and let $d = d_{t-1}$  and $v = v_t$. 

To bound the change $\Delta \Phi$, for any $a, b \in \BR$ satisfying $|a-b| \le 1$, by Taylor series expansion of $f(r)=\exp(\lambda^2r^2)$, we have
\begin{align*}
    \ f(a)-f(b) & \le  2\lambda^2~ bf(b) (a-b) + \frac{1}{2} \cdot 2\lambda^2~f(b)(2\lambda^2 b^2 + 1) (a-b)^2 +  \frac16 \cdot \max_{r \in [a,b]}|f'''(r)|(a-b)^3 \\
    \ & \le 2\lambda^2 bf(b) (a-b) + 4\lambda^4 b^2 f(b)(a-b)^2 + 2\lambda^2f(b)(a-b)^2 + \text{Remainder}.
\end{align*}
\mnote{This seems like a big problem. Don't see how to control the remainder term. The outliers may dominate it completely.}

\hnote{
We can write $\exp(\lambda^2(r + \Delta r)^2)$ as $\exp(\lambda^2(r + \Delta r)^2) = \exp(\lambda^2 r^2 + \lambda^2 r \Delta r + \lambda^2 \Delta r^2)$.  
We have $|\Delta r| \leq 1$. Let's imagine $\lambda = 1/\log(T)$, then $r$ is roughly $\log^{3/2}(T)$, so we can expect the change in the exponent $\lambda^2 r \Delta r + \lambda^2 \Delta r^2$ to be less than $1$? 
For the outliers, maybe the hope is that the tail probability cancels out the exponent growth? 
}

\begin{align*}
    \  \cosh(\lambda a) - \cosh(\lambda b) &=  \lambda \sinh(\lambda b) \cdot (a-b)  + \frac{\lambda^2}{2!} \cosh(\lambda b) \cdot (a-b)^2 + \frac{\lambda^3}{3!} \sinh(\lambda b)\cdot (a-b)^3 + \cdots , \\[0.8ex]
    \                & \le  \lambda \sinh(\lambda b)  \cdot(a-b) + \lambda^2 \cosh(\lambda b)  \cdot(a-b)^2,\\[1.1ex]
    \   & \le  \lambda \sinh(\lambda b)  \cdot(a-b) + \lambda^2 |\sinh(\lambda b)|  \cdot(a-b)^2 + \lambda^2(a-b)^2,
\end{align*}
where the first inequality follows since $|\sinh(a)| \le \cosh(a)$ for all $a \in \BR$, and since $|a-b|\le 1$ and $\lambda < 1$, so the higher order terms in the Taylor expansion are dominated by the first and second order terms. The second inequality uses that $\cosh(a) \le |\sinh(a)|+1$ for $a \in \BR$.

After choosing the sign $\chi_t$, the discrepancy vector $d_t = d + \chi_t v$. Defining $s_{k}(x) = \sinh(\lambda \cdot d^T\tM_k x)$ and noting that $|v^T \tM_k x| \le 1$, the above upper bound on the Taylor expansion gives us that 
\begin{align*}
    \ \Delta\Phi &\le \chi_t \left (\sum_{k = 0}^{\kappa} \lambda ~\BE_{x}\left[ s_{k}(x)  v^T\tM_k x\right]\right) + \sum_{k = 0}^{\kappa} \lambda^2 ~\BE_{x}\left[|s_{k}(x)| \cdot  x^T\tM_kvv^T\tM_kx\right] + \sum_{k = 0}^{\kappa} \lambda^2~\BE_{x}\left[ x^T\tM_kvv^T\tM_kx\right]\\
    \ &:= \chi_t L + Q + Q_*.
\end{align*}
where $L, Q$ and $Q_*$ denote the first, second and third terms respectively.

Since, our algorithm uses the greedy strategy, choosing $\chi_t$ to be the sign that minimizes the potential, and taking expectation over the incoming vector $v$, we get
\begin{align*}
    \ \BE_{v}[\Delta\Phi] &\le -\BE_{v}[|L|] + \BE_{v}[Q] + \BE_{v}[Q_{*}].\\
\end{align*}

We will prove the following upper bounds on the quadratic (in $\lambda$) terms $Q$ and $Q_*$.
\begin{claim}\label{claim:gen-quadratic}
$ \BE_{v}[Q] \le 2\lambda^2 \sum_{k=0}^{\kappa} 2^{-k} ~\BE_{x}[|s_{k}(x)|]$ and $\BE_{v}[Q_*] \le 4\lambda^2.$
\end{claim}

On the other hand, we will show that the linear (in $\lambda$) term $L$ is also large in expectation.
\begin{claim}\label{claim:gen-linear}
$ \BE_{v}[|L|] \ge \lambda B^{-1} \sum_{k=0}^{\kappa} 2^{-k} ~ \BE_{x}[|s_{k}(x)|] - 1$ where $B = \kappa \log(\Phi^2 nT).$
\end{claim}

By our assumption $\Phi \ge T$, so it follows that $2\lambda \le B^{-1}$. Therefore, combining the above two claims, we get that 
$$\BE_{v}[\Delta \Phi] \le (2\lambda^2-\lambda B^{-1}) \left(\sum_{k=0}^{\kappa} 2^{-k} ~ \BE_{x}[|s_{k}(x)|]\right) + 1 + 4\lambda^2 \le 2.$$

This finishes the proof of Lemma \ref{lemma:gen-drift} assuming the claims which we prove next.
\end{proof}

\begin{proof}[Proof of Claim \ref{claim:gen-quadratic}]
Recall that $\BE_{v}[vv^T] = \cov$ which satisfies $\tM_k \cov \tM_k = 2^{-k} \tM_k $ and $\Pi_k \preccurlyeq \tM_k \preccurlyeq 2\Pi_k$. Therefore, using linearity of expectation,
\begin{align*}
    \ \BE_{v}[Q] &= \sum_{k=0}^{\kappa} \lambda^2 ~ \BE_{x}[|s_{k(x)}| \cdot x^T\tM_k \cov \tM_k x] = \lambda^2 \sum_{k=0}^{\kappa}  2^{-k} ~ \BE_{x}[|s_{k}(x)| \cdot x^T \tM_k x]\\
    \ &\le 2\lambda^2 \sum_{k=0}^{\kappa} 2^{-k} ~ \BE_{x}[|s_{k}(x)|],
\end{align*}
where the last inequality uses that $x^T \tM_k x \le \|\tM_k\|_{\op}\|x\|_2^2 \le 2$ for all $x$ in the support of $q$. 

Similarly, we may bound 
\[ \BE_{v}[Q_{*}] = \sum_{k = 0}^{\kappa} \lambda^2~\BE_{x}\left[ x^T\tM_k\cov\tM_kx\right]  \le 2\lambda^2 \sum_{k=0}^{\kappa} 2^{-k} \le 4\lambda^2.\qedhere\]
\end{proof} 

\vspace*{10pt}

\begin{proof}[Proof of Claim \ref{claim:gen-linear}]


To lower bound the linear term, we use the fact that $|L(v)| \ge {\|f\|^{-1}_{\infty}} \cdot f(v) \cdot L(v)$ for any real-valued non-zero function $f$. We will choose the function $f(v) = d^T\tM v \cdot \ind_{\CG}(v)$ where $\CG$ will be the event that $|d^T\tM v|$ is small which we know is true because of Lemma \ref{lemma:tail}.\\

In particular, set $\delta^{-1} = 2\kappa (n\Phi) \log(4n \Phi)$ and let $\CG$ denote the event that $\lambda|d_t^T \tM_k v| \le \log (4 \Phi/\delta)$ for every $k \le \kappa$. Recalling that $\tM = \sum_{k=0}^{\kappa} \tM_k$, when the event $V \in \CG$ occurs, then $\lambda |d^T \tM v| \le \kappa \log (4 \Phi/\delta) := B$. Then, $f(v) = d^T\tM v \cdot \ind_{\CG}(v)$ satisfies $\|f\|_\infty \le \lambda^{-1} B$, and we can lower bound,
\begin{align}\label{eqn:lterm}
    \ \BE_{v}[|L|] &\ge \frac{\lambda}{B} \sum_{k=0}^{\kappa} \lambda ~  \BE_{vx} [s_{k}(x) \cdot d^T \tM v \cdot v^T \tM_k x\cdot \ind_{\CG}(v)] \notag \\
    \ &= \frac{\lambda^2}{B} \sum_{k=0}^{\kappa} \BE_{x} [s_{k}(x) \cdot d^T \tM \cov \tM_k x] - \frac{\lambda^2}{B} \sum_{k=0}^{\kappa} \BE_{x} [s_{k}(x) \cdot d^T \tM \cov_\err \tM_k x],
\end{align}
where $\cov_\err = \BE_{v}[vv^T \ind_{\comp\CG}(v)]$ satisfies $\|\cov_\err\|_{\op} \le \sfp(V \notin \CG) \le \delta$ using Lemma \ref{lemma:tail}.\\

To bound the first term in \eqref{eqn:lterm}, recall that $s_k(x) = \sinh(\lambda d^T \tM_k x)$. Using $\tM \Sigma \tM_k = 2^{-k} \tM_k$ and the fact that $\sinh(a)a \ge |\sinh(a)| - 2$ for any $a \in \BR$, we have  
\begin{align*}
    \lambda ~\BE_{x} [s_{k}(x) \cdot d^T \tM \cov \tM_k x] = 2^{-k} ~\BE_{x} [s_{k}(x) \cdot \lambda d^T \tM_k x] \ge 2^{-k}~ \left(\BE_{x} [|s_{k}(x)|] - 2\right).
\end{align*}

While the second term can be upper bounded by using the bounds on the operator norm of the matrices $\tM_k$  and $\cov_\err$. In particular, we have that $|d^T \tM \cov_\err \tM_k x | \le 2\|\tM d\|_2\|x\|_2 \le 2\delta \|\tM d\|_2$. Since $\tM \preccurlyeq \sum_{k=0}^\kappa \Pi_k$, using Lemma \ref{lemma:tail}, it follows that  $\|\tM d\|_2 \le \kappa n \lambda^{-1}\log(4n \Phi)$ and by our choice of $\delta$, $$\lambda |d^T \tM \cov_\err \tM_k x| \le 2\delta\kappa n \log(4n \Phi) = \Phi^{-1}.$$

Plugging the above bounds in \eqref{eqn:lterm}, 
\begin{align*}
    \BE_{p(v)}[|L|] &\ge  \frac{\lambda}{B} \sum_{k=0}^\kappa 2^{-k} ~\left(\BE_{x} [|s_{k}(x)|] - 2\right) -  \frac{\lambda}{B} \cdot \Phi^{-1} \left( \sum_{k=0}^{\kappa}  \BE_x[|s_k(x)|] \right) \\ 
    &\ge  \frac{\lambda}{B} \sum_{k=0}^\kappa 2^{-k} ~\BE_{x} [|s_{k}(x)|] - \frac{\lambda}{B} \sum_{k=0}^\kappa 2^{-k+1} - \frac{\lambda}{B}\\
    \ & \ge \frac{\lambda}{B} \sum_{k=0}^\kappa 2^{-k} ~\BE_{x} [|s_{k}(x)|] - 1,
\end{align*}
where the second inequality follows since $\sum_{k=0}^\kappa \BE_x[|s_k(x)|] \le \Phi.$
\end{proof}


\newpage

For brevity, let $d \equiv d(t-1)$ be the discrepancy vector at time step $t-1$, $v \equiv v(t)$ be the input vector at time $t$ and $a_{k}(x) = \exp((\alpha \cdot d^T\widetilde{M}_k x)^2)$. Let us also assume that $\|d\|_2 \le T$.\\

First we note by taylor expansion, that for $f(r)=e^{\alpha^2 r^2}$, for any $\delta$ satisfying $|\delta| <  1$, it holds that
\begin{align*}
    \ f(r+\delta) - f(r) & \le  2\alpha^2 rf(r) \delta + \frac12 \cdot 2\alpha^2f(r)(2\alpha^2 r^2 + 1) \delta^2 + \ldots \\
    \ & \le 2\alpha^2 rf(r) \delta + 4\alpha^4 r^2 f(r)\delta^2 + 2\alpha^2f(r)\delta^2.
\end{align*}


Since $d(t) = d + \eps_v v$, using the above, we can write
\begin{align*}
    \ \Delta\Phi &\le \eps_v \left(\sum_{k = \smin}^{\smax} 2\alpha^2 \cdot \BE_{q(x)}\left[ a_{k}(x) d^T\widetilde{M}_k x \cdot v^T\widetilde{M}_k x\right]\right) + \sum_{k = \smin}^{\smax} 4\alpha^4 \cdot \BE_{q(x)}\left[a_k(x) \cdot  (d^T\widetilde{M}_k x)^2 (v^T\widetilde{M}_k x)^2\right] \\
    \ & \qquad + \sum_{k = \smin}^{\smax} 2\alpha^2 \cdot \BE_{q(x)}\left[ a_k(x) (v^T\widetilde{M}_k x)^2\right]\\
    \ &:= \eps_v L + Q_1 + Q_2.
\end{align*}

Choosing $\eps_v$ to be the sign that minimizes the potential, and taking expectation over the incoming vector $v$, we get
\begin{align*}
    \ \BE_v[\Delta\Phi] &\le -\BE_v[|L|] + \BE_v[Q_1] + \BE_v[Q_2].\\
\end{align*}

\textbf{Quadratic Term $Q_1$:} Noting that $\widetilde{M}_k \cov \widetilde{M}_k = 2^{-k} \widetilde{M}_k $ and that $\Pi_k \preccurlyeq \widetilde{M}_k \preccurlyeq 2\Pi_k$, we get
\begin{align*}
    \ \BE_{p(v)}[Q_2] &= \sum_{k=\smin}^{\smax} 4\alpha^4 \cdot \BE_{q(x)}[a_{k}(x) \cdot (d^T\widetilde{M}_k x)^2 \cdot x^T\widetilde{M}_k \cov \widetilde{M}_k x] = 4\alpha^4 \sum_{k=\smin}^{\smax}  2^{-k} \cdot \BE_{q(x)}[a_{k}(x) \cdot (d^T\widetilde{M}_k x)^2  \cdot x^T \widetilde{M}_k x]\\
    \ &\le 8\alpha^4 \sum_{k=\smin}^{\smax} 2^{-k} \cdot \BE_{q(x)}[a_{k}(x) \cdot (d^T\widetilde{M}_k x)^2 ],
\end{align*}
where in the last line we used that $\|x\|_2^2 \le 1$ for all $x$ in the support of $q$.\\

\textbf{Quadratic Term $Q_2$:} Similarly, we have
\begin{align*}
    \ \BE_{p(v)}[Q_1] &= \sum_{k=\smin}^{\smax} 2\alpha^2 \cdot \BE_{q(x)}[a_{k}(x) \cdot x^T\widetilde{M}_k \cov \widetilde{M}_k x] = 2\alpha^2 \sum_{k=\smin}^{\smax}  2^{-k} \cdot \BE_{q(x)}[a_{k}(x) \cdot x^T \widetilde{M}_k x]\\
    \ &\le 4\alpha^2 \sum_{k=\smin}^{\smax} 2^{-k} \cdot \BE_{q(x)}[a_{k}(x)].
\end{align*}

\textbf{Linear Term: } Recall that $\widetilde{M} = \sum_{k=\smin}^{\smax} \widetilde{M}_k$. To bound the linear term, we first notice that when $v \in \CG$, then $|d^T \widetilde{M} v| \le \sum_{k=\smin}^{\smax} \frac{\sqrt{4\log \phi}}{\alpha} \le \frac{2\log^{3/2} (nT)}{\alpha}$. Using that $|L(v)| \ge \frac{f(v)}{\|f\|_{\infty}} L(v)$ for any real-valued function $f$, and choosing $f(v) = d^T\widetilde{M} v \cdot \ind_{\CG}(v)$, we get that
\begin{align*}
    \ \BE_{p(v)}[|L|] &\ge \frac{\alpha^3}{2\log^{3/2} (nT)} \sum_{k=\smin}^{\smax}  \BE_{p(v)q(x)} [a_{k}(x) \cdot (d^T \widetilde{M}_k x) (x^T \widetilde{M}_k v) (v^T  \widetilde{M} d) \ind_{\CG}(v)] \\
    \ &= \frac{\alpha^3}{2\log^{3/2} (nT)} \sum_{k=\smin}^{\smax}\BE_{q(x)} [a_{k}(x) \cdot d^T \widetilde{M}_k x x^T \widetilde{M} \cov' \widetilde{M}_k d],
\end{align*}
%{\bf NB:} {\em In the first line, it should be $d^T\tilde{M}_k x x^T \tilde{M}_k v v^T \tilde{M} v$ ?
%(So $M_k$ instead of M in first product, and $M$ instead of $M_k$ in third product).
%In second line, $M$ instead of $M_k$ in last product.}\\

where $\cov' = \cov - A$ with $A = \BE_{p(v)}[vv^T \cdot \ind_{\comp\CG}(v)]$ satisfying $0 \preccurlyeq A \preccurlyeq \beta I$ for $\beta = \poly((nT)^{-1})$.\\



Now, $\|\Sigma - \Sigma'\|_{op} \leq \beta$. Thus, $|d^T \widetilde{M} x x^T \widetilde{M}_k (\Sigma' - \Sigma) \widetilde{M} d | \le \|d\|^2_2\|x\|^2_2 = O(T^2 \beta) = T^{-3}$ choosing $\beta$ appropriately. Further, $\widetilde{M} \Sigma \widetilde{M}_k = 2^{-k} \widetilde{M}_k$. Using this, we have 

%{\bf NB:} {\em Similarly in the line above. The $M_k$'s and $M$'s seem to be swapped}\\


\begin{align*}
    \BE_{p(v)}[|L|] &\ge \frac{\alpha^3}{4\log^{3/2} (nT)} \sum_{k=\smin}^{\smax} 2^{-k} \cdot   \BE_{q(x)} [a_{k}(x) \cdot (d^T\widetilde{M}_k x)^2] - \frac{\Phi(d)}{T^2}.
\end{align*}

\paragraph{Small Drift.}
Collecting all the terms above, we get 
\begin{align}\label{eqn:1}
    \BE_v[\Delta \Phi] \le \frac{\Phi(d)}{T^2} + \left(-\frac{\alpha^3}{\log^{3/2} (nT)} + 8 \alpha^4\right) \sum_{k=\smin}^{\smax} 2^{-k}\BE_{q(x)}[a_k(x) (d^T \widetilde{M}_k x)^2] + 4\alpha^2 \sum_{k=\smin}^{\smax} 2^{-k}\BE_{q(x)}[a_k(x)].
\end{align}

Let us set $\alpha = 1/(100\log^{3/2}(nT))$, so that the second term above is negative since 
$$ \left(-\frac{\alpha^3}{\log^{3/2} (nT)} + 8 \alpha^4\right) \le -\frac{\alpha^3}{2\log^{3/2} (nT)}.$$

Further, note that $\exp(\alpha^2 (d^T M_k x)^2) \le e$ when $|d^T\widetilde{M}_kx| \le 1/\alpha$. Therefore,
\begin{align*}
    \ \sum_{k=\smin}^{\smax} 2^{-k}\cdot \BE_{q(x)}[a_k(x) (d^T \widetilde{M}_k x)^2] &\ge \sum_{k=\smin}^{\smax}   2^{-k} \cdot \frac1{\alpha^2} \cdot \left(\BE_{q(x)}[a_k(x)] - \BE_{q(x)}\left[a_k(x) \cdot \ind_{|d^T \widetilde{M}_k x| \le \frac1\alpha}\right]\right) \\
    \ & \ge \sum_{k=\smin}^{\smax}   2^{-k} \cdot \frac1{\alpha^2} \cdot  \left(\BE_{q(x)}[a_k(x)] - e\right).
\end{align*}

Plugging the above in \eqref{eqn:1}, we get that
\begin{align*}
    \BE_v[\Delta \Phi] \le \frac{\Phi(d)}{T^2} + O(1) +  \left(-\frac{\alpha}{2\log^{3/2} (nT)} + 4\alpha^2\right)  \sum_{k=\smin}^{\smax} 2^{-k}\BE_{q(x)}[a_k(x)].
\end{align*}
One can check that for our previous choice of $\alpha = 1/(100\log^{3/2}(nT))$, we have that $$\left(-\frac{\alpha}{2\log^{3/2} (nT)} + 4\alpha^2\right) \le 0$$ and hence,
\[ \BE_{p(v)}[\Delta\Phi] \le \frac{\Phi(d)}{T^2} + O\left(1\right).\]

Therefore, with high probability, the potential is bounded by $\poly(nT)$ at time $T$.


\section{Discrepancy with respect to Arbitrary Convex Bodies}
\label{sec:banasczyck}






\subsection{Discrepancy Bound}



For a set $T \subseteq \BR^n$, let $w(T) = \BE_G[\sup_{t \in T} \ip{G}{t}]$ denote the Gaussian width of $T$. Note that the gaussian width is $ \Theta(\sqrt{n})$ factor larger than the spherical width $\BE_\theta[\sup_{t \in T} \ip{\theta}{t}]$ where $\theta$ is randomly chosen from the unit sphere $\BS^{n-1}$. Let $\diam(T) $ denote the diameter of the set $T$.

\begin{lemma} Let $K \subseteq \BR^n$ be a symmetric convex body with $\gamma_n(K) \ge 1/2$ and $G \in \BR^n$ be a standard Gaussian. Then, $w(K^\circ)  \le \frac{3}{2}$. Moreover, $\diam(K^\circ) \le 2$.
\end{lemma}

Let $\CN(T, \eps)$ denote the size of the smallest $\eps$-net of $T$ in the Euclidean metric, \emph{i.e.}, the smallest number of closed balls of radius $\eps$ whose union covers $T$.

\begin{lemma}[Sudakov minoration] For any set $T \subseteq \BR^n$ and any $\eps > 0$
\[ w(T) \gtrsim \eps \sqrt{\log \CN(T,\eps)}.\]
\end{lemma}


%\begin{lemma}[Two-sided Sudakov's inequality] For any set $T \subseteq \BR^n$, let $\smax = \log \lceil \frac{4\sqrt{n}}{w(T)} \rceil$ and $\smin = \log \lceil 1/\diam(T) \rceil$. Then, we have that
%\[ \max_{k \in [\smin, \smax]} 2^{-k}  \sqrt{\log \CN(T,2^{-k})} \lesssim w(T) \lesssim \sum_{k=\smin}^{\smax} 2^{-k}  \sqrt{\log \CN(T,2^{-k})}.\]
%\end{lemma}

Given a convex body $K^\circ$, let $\smax = \lceil 4\log T \rceil$ be the finest scale and $\smin = \log \lceil 1/\diam(K^\circ) \rceil$ be the coarsest scale. (Note that $\smin \ge -1$ because of the lemma above).  Let $T_k$ denote an optimal $2^{-k}$-net of $K^\circ$ where $k \in \{\smin, \cdots, \smax\}$. \\

Define the following layered graph (not a tree) where we index the layers starting from $\smin$: the first layer labeled with index $\smin$ consists of the origin and the vertices of layer $k$ are elements of $T_{k}$. There is an edge between $u \in T_k$ and $v \in T_{k+1}$ iff $v \in B(u,2^{-k})$ where $B(u,r)$ denotes the euclidean ball of radius $r$ centered at $u$. We identify an edge $(u,v)$ with the vector $u-v$ and define its length as $\|u - v\|$. Let $E_k$ denote the edges between layer $k$ and $k+1$. Note that $|E_k| \le |T_{k+1}|^2 \le \CN(K^\circ, 2^{-k-1})^2$ and any $e \in E_k$ has length at most $2^{-k}$.



In our potential we will choose $y$ by first sampling an integer $k$ uniformly in $[\smin, \smax]$  and then taking $y$ uniform in $2^k E_k$. Note that $\|y\|_2 \le 1$. Suppose that  the quadratic potential is bounded by $\phi$. Set $M = \frac{\sqrt{\log \phi}}{\alpha}$. Then, we have that for any layer $k$ and any edge $e \in E_k$,
\[\ip{d}{e} \lesssim M \cdot 2^{-(k+1)} \sqrt{\log |T_{k+1}|} = c M \cdot 2^{-(k+1)} \sqrt{\log \CN(K^\circ, 2^{-{k+1}})}.\]

Let $e_{\smin}, \ldots, e_{\smax}$ denote the edges along any path from the origin to $v \in T_{\smax}$ and note that $v = \sum_{k=\smin}^{\smax} e_i$. Then, for any $d \in \BR^n$ with $\|d\|_2 \le T$, we have that  
\begin{align*}
    \ \sup_{y \in K^\circ} \ip{d}{y} &\le \sup_{v \in T_{\smax}} \ip{d}{v} +  o(1) \\ 
    \ & \le (\smax - \smin) \cdot M \cdot \left(\max_k 2^{-(k+1)} \sqrt{\log \CN(K^\circ, 2^{-{k+1}})}\right)  +  o(1) \\
    \ & \le c w(K^\circ)\log T \cdot M = O(M \log T) = O(\log^3 T).
\end{align*}


\newpage 



==> isotropic.tex <==
\section{Discrepancy for Isotropic Convex Bodies}
\label{sec:isotropic}


We say that a symmetric convex body $K \subseteq \BR^n$ is \emph{dual isotropic} if the covariance matrix for the uniform distribution on $K^\circ$ is the identity matrix $I_n$. In this scenario, we also call the polar body $K^\circ$ isotropic. 

We remark that this is not the usual notion of the isotropic position of a convex body as we do not require $K^\circ$ to be of unit volume. 

In this section, we prove the following. 

\mnote{This proof does not work at the moment}

\begin{theorem}\label{thm:iso-disc}
    Let $K \subseteq \BR^n$ be a symmetric convex body such that $K/n$ is dual isotropic. Let be a distribution supported over vectors with Euclidean norm at most $1$ in $\BR^n$. Then, for vectors $v_1, \ldots, v_T$ sampled i.i.d. from $\sfp$, there is an online algorithm that  w.h.p. maintains discrepancy a discrepancy vector $d_t$ satisfying $\|d_t\|_K = O(\log^6(nT))$ at all times $t \in [T]$.
\end{theorem}

Note that the scaling above is chosen to compare it to the Komlos and Banasczyck setting.

\subsection{Preliminaries on Isotropic Convex Bodies and Log-concave Measures}

For a linear subspace $H \subseteq \BR^n$ and a convex body $K \subseteq H$, we say that $K$ is dual isotropic with respect to $H$ if the covariance matrix of $K$ is $\Pi_H$ where $\Pi_H$ is the orthogonal projection on to the subspace $H$.

\begin{proposition} \label{prop:isotropic}
    Let $K \subseteq \BR^n$ be a symmetric convex body that is dual isotropic, and let $H \subseteq \BR^n$ be a linear subspace. Then, $K\cap H$ is dual isotropic with respect to $H$.
\end{proposition}
\begin{proof}
    Let $X$ be drawn uniformly from $K^\circ$, so that $Y=\Pi_HX$ is uniform over $(K \cap H)^\circ$. Then the covariance matrix of $Y$ is  given by 
    \[ \BE_y[yy^T] = \BE_x[\Pi_H xx^T \Pi_H] = \Pi_H \cdot I_n \cdot \Pi_H = \Pi_H. \qedhere\]
\end{proof}

Isotropic bodies are approximated by balls as the following proposition shows.
\begin{proposition}[\cite{KLS95}]
    \label{prop:kls}
    If $K \subseteq \BR^n$ is a dual isotropic convex body, and $B$ is the unit Euclidean ball, then
    \[ \sqrt{\frac{n+2}{n}}B \subseteq K^\circ \subseteq \sqrt{n(n+2)}B.\]
\end{proposition}

\begin{lemma}\label{lemma:john}
Let $K \subseteq \BR^n$ be a dual isotropic convex body. Then, for any vector $d \in \BR^n$,
\begin{align*}
    \p_{y \sim K^\circ}\left[\ip{d}{y} \geq \frac12 \|d\|_K\right] \geq n^{-2n}. 
\end{align*}
\end{lemma}
\newcommand{\Cov}{\mathsf{Cov}}
\begin{proof}
\mnote{To be simplified and notation to be updated}
The following sandwiching condition is by John's theorem:
\begin{align*}
    E(\Cov(K^\circ)^{-1}) \subseteq K^\circ \subseteq \sqrt{n} \cdot E(\Cov(K^\circ)^{-1}),
\end{align*}
where $E(A) = \{y: y^\top A y \leq 1\}$. 
Let $v = d / \norm{d}_2$ be the unit vector in the direction of $d$.
We consider cross-sections of $K^\circ$ of the form $K^\circ \cap (v^\perp + t v)$, whose $(n-1)$-dimensional volume is denoted as $g_{K,v}(t)$.  
The largest $t_{\max}$ that satisfies $K^\circ \cap (v^\perp + t_{\max} \cdot v) \neq \emptyset$ gives an extreme point $x_d$ (this might be a face of $K$ but the proof is the same) of $K^\circ$ such that $\langle d, x_d \rangle = 1$. 
We are interested in ratio between the volume of $K \cap (\cup_{t \geq t_{\max}/2} (v^\bot + tv))$ and the volume of $K$.  

We note that the cone formed by $x_d$ and $K \cap v^\bot$ (the cross-section through the centroid) lies in $K$, having volume at least $\frac{1}{2n}$ times the volume of the inscribed ellipsoid (the factor $n$ comes from enlarging the cone to a cylinder, which has volume at least half of the inscribed ellipsoid). 
This proves that the top $1/2$ height of the cone has volume at least $\frac{1}{2n \cdot 2^n}$ times the volume of the inscribed ellipsoid, which is at least $\frac{1}{2n \cdot 2^n \cdot \sqrt{n}^n}$ times the volume of $K$. 
This proves the lemma. 
\end{proof}

\paragraph{Log-concave Measures}
A probability measure $\sfp$ on $\BR^n$ is called log-concave if for all non-empty measurable sets $\SA, \SB \subseteq \BR^n$ and for all $0< \lambda < 1$, we have 
\[ \sfp(\lambda \SA + (1-\lambda)\SB) \ge \sfp(\SA)^\lambda\sfp(\SB)^{1-\lambda}.\]

It is well-known that the uniform distribution on a convex body is log-concave. Log-concavity is preserved under affine transformations and taking marginals (c.f. \cite{LV07} Theorem 5.1). 

Log-concave distributions on the real line are sub-exponential (see Lemma 5.7 and Theorem 5.22 in \cite{LV07}) and in particular, \pref{prop:logconcave} also holds for log-concave probability distributions on $\BR$.

\subsection{Potential Function and Algorithm}

Our algorithm will use a similar greedy strategy as before with a suitable test distribution $\sfp_z$  that will be chosen later. Let $(\Sigma, (\Pi_k)_k, (M_k)_k)$ be the covariance decomposition of $\sfp$. Define the noisy distribution $\sfp_x = \sfp/2 + \sfp_z/2$.

At any time step $t$, let $d_{t} = \chi_1 v_1 + \ldots + \chi_t v_t$ denote the current discrepancy vector after the signs $\chi_1, \ldots, \chi_t \in \{\pm1\}$ have been chosen. Set $\lambda^{-1} = 12\log^2(nT)$, and define the potential 
\[ \Phi_t = \Phi(d_t) :=  \sum_{k=0}^{\kappa} \BE_{x\sim \sfp_x}\left[\exp\left(\lambda ~d_{t}^\top \tM_k x \right)\right].\]

When the vector $v_t$ arrives, the algorithm chooses the sign $\chi_t$ that minimizes the increase $\Phi_t - \Phi_{t-1}$.

\paragraph{Test Distribution.} To complete the description of the algorithm, we need to choose a suitable distribution on test vectors to give us control on the norm $\|\cdot\|_K = \sup_{y \in K^\circ} \ip{\cdot}{y}$. 

As before, let us denote by $H_k = \im(\Pi_k)$ the linear subspace that is the image of the projection matrix $\Pi_k$ where the subspaces $\{H_k\}_{k \le \kappa}$ are orthogonal and span $\BR^n$. Let us denote by $K_k = K \cap H_k$ the slice of the convex body $K$ with the subspace $H_k$. \pref{prop:isotropic} implies that the dual polar bodies $K^\circ_k := (K_k)^\circ = \Pi_k (K^\circ)$ are also in the dual isotropic position with respect to the corresponding subspace $H_k$.

Pick the final test distribution as $\sfp_z = \sfp_\cov/2 + \sfp_y/2$ where $\sfp_\cov$ and $\sfp_y$ denote the distributions given in \figref{fig:iso-test}. 
\begin{figure}[!h]
\begin{tabular}{|l|}
\hline
\begin{minipage}{\textwidth}
\vspace{1ex} 
\begin{enumerate}[(a)]
    \item $\sfp_\cov$ is uniform over the eigenvectors of the covariance matrix $\cov$.
    \item $\sfp_y$ samples a random vector as follows: pick an integer $k$ uniformly from $[0,\kappa]$ and choose a uniform vector from $r nK^\circ_k$ where the polar body $nK^\circ$ is isotropic and $r=1/C\log(nT)$.
\end{enumerate}
\vspace{0.1ex}
\end{minipage}\\
\hline
\end{tabular}
\caption{Test distributions $\sfp_\cov$ and $\sfp_y$}
\label{fig:iso-test}
\end{figure}

As before, adding the eigenvectors will allows us to control the Euclidean length of the discrepancy vectors in the subspaces $H_k$ as they form an orthonormal basis for these subspaces. And similar to previous section, the test vectors chosen above may have large Euclidean length. In particular, \pref{prop:kls} implies that any vector in the support of $y$ has Euclidean norm at most $O(n)$.

The test distribution $\sfp_z$ is useful because of the following lemma.

\begin{lemma} \label{lemma:isotropic}
At any time $t$, if $\Phi_t \le T$, then we have that 
\[ \|\Pi_kd\|_2 \le \sqrt{\lambda^{-1}\dim(H_k)\log(nT)} ~\text{ and }~ \|d\|_K \le \log^6(nT).\]
\end{lemma}
\begin{proof}
The first statement is the same as that of \lref{lemma:chaining}. To see the bound on $\|d\|_K$, since $\tM_k M = \Pi_k$, our choice of the test distribution gives us the following for every $k$,
\[ \sup_{y \in K^\circ_k} \exp\left( \lambda r n  \cdot |d^\top\Pi_k y |\right) ~\le~ n^{\dim(H_k)} 4\kappa \Phi,\]
where the second inequality follows from \lref{lemma:john}.

Therefore, $|d^\top \Pi_k y| \le (r\lambda)^{-1}\log^2(nT) \le \log^5(nT)$ for every $k$ and hence
\[ \|d\|_K = \sup_{y \in K^\circ} \ip{d}{y} \le \sum_{k=0}^\kappa \sup_{y \in K^\circ_k} \ip{d}{\Pi_k y} = \log^6(nT). \qedhere\]
\end{proof}

The next lemma shows that most of the times the expected increase (or drift) in the potential is small.

\begin{lemma}[Bounded Positive Drift]\label{lemma:iso-drift} If at any time $t$, it holds that $ \Phi_{t-1} \le T$, then there exists an event $\CE_t$ such that 
\[\BP_{v_t \sim \sfp}(\CE_t) \ge 1-T^{-4} ~\text{  and } ~\BE_{v_t \sim \sfp}[\Phi_t \cdot \ind_{\CE_t}] - \Phi_{t-1} = O(1).\] 
\end{lemma}

By a union bound and a truncation argument as used in the previous proofs, this implies that w.h.p. the potential $\Phi_t \le 3T^5$ for every $t \in [T]$. Combined with \lref{lemma:isotropic}, this proves \thmref{thm:iso-disc}. 

We prove \lref{lemma:iso-drift} in the next section.

\subsection{Drift Analysis: Proof of \lref{lemma:iso-drift}} We first note the following tail bound analogous to \lref{lemma:tail} and \lref{lemma:gen-tail-ban}. Let $\CG_t = \CG(d_t)$ denote the set of vectors in the support of $\sfp$ such that $\lambda |d_t^\top \tM_k v| \le \log (4\kappa \Phi_t/\delta)$ for every $k \le \kappa$. 

\begin{lemma}\label{lemma:iso-tail}
For any $\delta > 0$, the following holds at any time $t$, $\BP_{v \sim \sfp}(v \notin \CG_t) \le \delta$.
\end{lemma}

\begin{proof}[Proof of \lref{lemma:iso-drift}]

Let us fix a time $t$. To simplify the notation, let $\Phi = \Phi_{t-1}$ and $\Delta\Phi = \Phi_t - \Phi$, and let $d = d_{t-1}$  and $v = v_t$. 

To bound the change $\Delta \Phi$, we use the following inequality, which follows from a modification of the Taylor series expansion of $\cosh(r)$ and holds for any $a,b \in \BR$,
\begin{align}\label{eqn:taylor}
    \ \cosh(\lambda a)-\cosh(\lambda b) & \le \lambda \sinh(\lambda b) \cdot (a - b) + \frac{\lambda^2}{2} \cosh(\lambda b) \cdot e^{|a-b|}(a - b)^2.
\end{align}
Note that when $|a-b| \ll 1$, then $e^{|a-b|} \le 2$, so one gets the first two terms of the Taylor expansion as an upper bound, but here we will also use it when $|a-b|\gg 1$.

Define the distribution $\sfp_w = \frac34 \sfp + \frac14p_\cov$ and note that the distribution $\sfp_x$ appearing in the potential $\Phi$ satisfies $\sfp_x = \frac34 \sfp_w + \frac14 \sfp_y$. Furthermore, observe that every vector in the support of $\sfp_w$ has Euclidean length at most $1$ while $y \sim \sfp_y$ may have large Euclidean length.

After choosing the sign $\chi_t$, the discrepancy vector $d_t = d + \chi_t v$. Defining $s_{k}(x) = \sinh(\lambda \cdot d^\top\tM_k x)$ and $c_{k}(x) = \cosh(\lambda \cdot d^\top\tM_k x)$ for any $x \in \BR^n$, \eqref{eqn:taylor} implies that $\Delta\Phi := \Delta\Phi_1 + \Delta\Phi_2$ where
\begin{align*}
    \ \Delta\Phi_1 &\le \chi_t \cdot \frac34\left (\sum_{k = 0}^{\kappa} \lambda ~\BE_{w}\left[ s_{k}(w)  v^\top\tM_k w\right]\right) + \frac34\sum_{k = 0}^{\kappa} \lambda^2 ~\BE_{w}\left[c_{k}(w) \cdot  w^\top\tM_kvv^\top\tM_kw\right] : = \chi_t L_1 + Q_1, \text{ and },\\
    \ \ \Delta\Phi_2 &\le \chi_t \cdot  \frac14\left (\sum_{k = 0}^{\kappa} \lambda ~\BE_{y}\left[ s_{k}(y)  v^\top\tM_k y\right]\right) + \frac14\sum_{k = 0}^{\kappa} \lambda^2 ~\BE_{y}\left[c_{k}(y) \cdot e^{\lambda |v^\top \tM_ky|} y^\top\tM_kvv^\top\tM_ky\right] : = \chi_t L_2 + Q_2.
\end{align*}

Since, our algorithm uses the greedy strategy, choosing $\chi_t$ to be the sign that minimizes the potential, and taking expectation over the incoming vector $v$, we get that for every $v$,
\begin{align*}
    \ \Delta\Phi &\le -|L_1 + L_2| + Q_1 + Q_2.\\
\end{align*}

Unlike before, we will not be able to prove that this potential always remains small in expectation, so let us define a good event $\CG:=\CG_t$ that $\lambda |d^T\Pi_k v| \le 12\log T$ for every $k$. Lemma \ref{lemma:iso-tail} implies that $\BP_v(\CG_t) \le T^{-4}$.

Given $v \in \BR^n$, let $P^\bot_v$ denote the projection on to the $(n-1)$-dimensional subspace orthogonal to $v$. We will prove the following upper bounds on the quadratic (in $\lambda$) terms $Q_1$ and $Q_2$.

\begin{claim}\label{claim:quadratic-ban}
$$\BE_{v}[(Q_1+Q_2)\cdot \ind_\CG] \le 4\cdot \lambda^2 \cdot \frac34\sum_{k=0}^{\kappa} 2^{-k} ~\BE_{w}[c_{k}(w)] + 4\cdot \lambda^2 \cdot \frac14\sum_{k=0}^{\kappa} ~\BE_{vy}[c_{k}(P^\bot_v y)\|\Pi_k v\|_2^2].$$
\end{claim}

On the other hand, we will show that the linear (in $\lambda$) terms $L_1 + L_2$ is also large in expectation.
\begin{claim}\label{claim:linear-ban}
  For a universal constant $C>0$ and some $B \le \kappa \log(\Phi^2 nT)$,
  $$\BE_{v}[|L_1 + L_2|\cdot \ind_{\CG}] \ge  \frac{\lambda}{B}\cdot \frac34\sum_{k=0}^\kappa 2^{-k}~~\BE_{w} [c_{k}(w)] + \frac{\lambda}{B}\cdot\frac14\sum_{k=0}^\kappa 2^{-k}~~\BE_{y} [c_{k}(y) |\lambda d^T \tM_k y|] - C.$$
\end{claim}

\mnote{How to argue the following from the above claims?}
By our assumption $\Phi \le T$, so it follows that $2\lambda \le B^{-1}$. Therefore, combining the above two claims,
$$\BE_{v}[\Delta \Phi \cdot \ind_\CG] \le C.$$
This finishes the proof of  \lref{lemma:gen-drift-ban} assuming the claims which we prove next.
\end{proof}
\vspace*{8pt}

To bound the drift, we need the following consequence of log-concavity of the test distribution $\sfp_y$.

\begin{lemma}\label{lemma:logconcave}
There exists a constant $C>0$, such that for every integer $k \le \kappa$, and every $v \in \im(\Pi_k)$, 
\[\BE_{y}\left[c_k(P^\bot_v y) \cdot \exp\left(s |v^T y|\right)|v^T y|^2\right]  \le C \cdot \BE_{y}\left[c_k(P^\bot_v y) \cdot \|v\|_2^2\right], \text{ for all } s \le \frac{\lambda^{-1}}{2\|v\|_2^2}.\]
\end{lemma}
\begin{proof}
    First note that as $v \in \im(\Pi_k)$, it suffices to assume that $y$ is uniformly drawn from $\lambda n K^\circ_k$ as otherwise the contribution is zero. Note that for any fixed value of $P^\bot_v y$, it still holds that $v^Ty$ is a scalar mean-zero log-concave random variable with variance 
    $$\sigma_v^2 := \BE_y[|v^\top y|^2] = v (\BE_y[yy^\top ]) v = \lambda\|v\|_2^2.$$
    
   Using Cauchy-Schwarz and \pref{prop:logconcave}, we get that for any fixed value of $P_v y$, 
    \begin{align*}
        \BE\left[e^{s |v^\top  y|} \cdot |v^\top y|^2\right] \le \sqrt{\BE\left[e^{2s |v^\top  y|}\right]} \cdot \sqrt{ \BE\left[|v^\top y|^4\right]} \le C \cdot \BE\left[|v^\top y|^2\right] \le C~\|v\|_2^2,
    \end{align*}
    where the expectation is over the scalar random variable $v^Ty$ conditioned on $P^\bot_v y$.
\end{proof}
\vspace*{8pt}

\begin{proof}[Proof of  \clmref{claim:quadratic-ban}]
Recall that $\BE_{v}[vv^\top] = \cov$ which satisfies $\tM_k \cov \tM_k = 2^{-k} \tM_k $ and $\Pi_k \preccurlyeq \tM_k \preccurlyeq 2\Pi_k$. Therefore, using linearity of expectation,
\begin{align}\label{eqn:int1}
    \ \BE_{v}[Q_1\cdot\ind_\CG] \le \BE_{v}[Q_1] &=\frac34 \sum_{k=0}^{\kappa} \lambda^2 ~ \BE_{w}[c_{k}(w) \cdot w^\top\tM_k \cov \tM_k w] = \lambda^2 \cdot \frac34 \sum_{k=0}^{\kappa}  2^{-k} ~ \BE_{w}[c_{k}(w) \cdot w^\top \tM_k w] \notag\\
    \ & \le 2\lambda^2 \cdot \frac34  \sum_{k=0}^{\kappa} 2^{-k} ~ \BE_{w}[c_{k}(w)\|w\|_2^2] \le 2\lambda^2 \cdot \frac34  \sum_{k=0}^{\kappa} 2^{-k} ~ \BE_{w}[c_{k}(w)].
\end{align}

To bound the term $\BE_v[Q_2 \cdot \ind_\CG]$, for a fixed $y \in \im(\Pi_k)$, let us decompose $y = \alpha_v \Pi_k v + P^\bot_v y$ where $\alpha_v = |v^T\Pi_ky|/{\|\Pi_k v\|^2_2}$. For any $v \in \CG$, we have that $\lambda |d^T \tM_k v| \le 12\log T$. Recall that $c_k(y) = \cosh(\lambda d^T\tM_k y)$ for any $k$ and that $\Pi_k \preccurlyeq \tM_k \preccurlyeq 2\Pi_k$. Therefore, using that $\cosh(a+b)\le \cosh(a)\cdot e^{|b|}$ for any $a,b \in \BR$, we obtain
\[ c_k(y)e^{\lambda|v^T\tM_ky|} \le c_k(P^\bot_v y)e^{2\lambda|d^T \Pi_k v|\alpha_v+2\lambda|v^T\Pi_k y|} \le c_k(P^\bot_v y) \cdot \exp\left(\frac{12\log T}{\|\Pi_k v\|_2^2}\cdot |v^T\Pi_k y|\right)  .\] 

Therefore, for any fixed $v \in \CG$, using \lref{lemma:logconcave}, 
\begin{align*}
    \ ~\BE_{y}\left[c_{k}(y) \cdot e^{\lambda |v^\top M_ky|} y^\top\tM_kvv^\top\tM_ky\right] &\le 4~ \BE_{y}\left[c_k(P^\bot_v y) \cdot \exp\left(\frac{12\log T}{\|\Pi_k v\|_2^2}\cdot |v^T\Pi_k y|\right)|v^T\Pi_k y|^2\right]\\
    \ & \le 4~ \BE_{y}\left[c_k(P^\bot_v y) \cdot \|\Pi_kv\|^2\right].
\end{align*}

Therefore, we may bound,
\begin{align}
    \ \BE_{v}[Q_2\cdot \ind_\CG] &\le 4 \cdot \lambda^2 \cdot  \frac14\sum_{k=0}^{\kappa} \BE_{y}[c_{k}(P^\bot_v y) \|\Pi_k v\|_2^2]. \notag\qedhere
\end{align}
\end{proof} 
\vspace*{8pt}

\begin{proof}[Proof of  \clmref{claim:linear-ban}]
Let $L = L_1 + L_2$. To lower bound the linear term, we proceed similar to the proof of \clmref{claim:linear} and use the fact that $|L(v)| \ge {\|f\|^{-1}_{\infty}} \cdot f(v) \cdot L(v)$ for any real-valued non-zero function $f$. We will choose the function $f(v) = d^\top\tM v \cdot \ind_{\CG}(v)$.\\

 Recalling that $\tM = \sum_{k=0}^{\kappa} \tM_k$, when the event $v \in \CG$ occurs, then $\lambda |d^\top \tM v| \le \kappa \log (4 \kappa\Phi/\delta) := B$. Then, $f(v) = d^\top\tM v \cdot \ind_{\CG}(v)$ satisfies $\|f\|_\infty \le \lambda^{-1} B$, and we can lower bound,
\begin{align}\label{eqn:lterm-iso}
    \ \BE_{v}[|L|\cdot \ind_\CG] &\ge \frac{\lambda}{\lambda^{-1} B} \cdot \frac34 \sum_{k=0}^{\kappa} \BE_{vw} [s_{k}(w) \cdot d^\top \tM v \cdot v^\top \tM_k w\cdot \ind_{\CG}(v)] + \frac{\lambda}{\lambda^{-1}B} \cdot \frac14\sum_{k=0}^{\kappa} \BE_{vy} [s_{k}(y) \cdot d^\top \tM v \cdot v^\top \tM_k y\cdot \ind_{\CG}(v)] \notag \\
    \ &= \frac{\lambda^2}{B} \cdot \frac34 \sum_{k=0}^{\kappa} \BE_{w} [s_{k}(w) \cdot d^\top \tM \cov \tM_k w] ~-~ \frac{\lambda^2}{B} \cdot \frac34 \sum_{k=0}^{\kappa} \BE_{w} [s_{k}(w) \cdot d^\top \tM \cov_\err \tM_k w] \notag \\
    \ &\qquad + \frac{\lambda^2}{B}  \cdot \frac14 \sum_{k=0}^{\kappa} \BE_{y} [s_{k}(y) \cdot d^\top \tM \cov \tM_k y] ~-~\frac{\lambda^2}{B}\cdot \frac14 \sum_{k=0}^{\kappa} \BE_{y} [s_{k}(y) \cdot d^\top \tM \cov_\err \tM_k y],
\end{align}
where $\cov_\err = \BE_{v}[vv^\top (1-\ind_{\CG}(v))]$ satisfies $\|\cov_\err\|_{\op} \le \BP_{v \sim \sfp}(v \notin \CG) := \delta$ where $\delta \le T^{-4}$ using  \lref{lemma:tail}.\\

To bound the terms involving $\cov$ in \eqref{eqn:lterm-iso}, we recall that $s_k(x) = \sinh(\lambda d^\top \tM_k x)$. Using $\tM \Sigma \tM_k = 2^{-k} \tM_k$ and the fact that $\sinh(a)a \ge \cosh(a)|a| - 2$ for any $a \in \BR$, we have  
\begin{align*}
    \lambda ~\BE_{w} [s_{k}(w) \cdot d^\top \tM \cov \tM_k w] ~=~ 2^{-k} ~\BE_{w} [s_{k}(w) \cdot \lambda d^\top \tM_k w] ~\ge~ 2^{-k}~ \left(\BE_{w} [c_{k}(w)|\lambda d^\top\tM_k w|] - 2\right),
\end{align*}
and similarly for $y$.

While the terms involving $\cov_\err$ can be upper bounded by using the bounds on the operator norm of the matrices $\tM_k$  and $\cov_\err$. In particular, we have that 
$$|d^\top \tM \cov_\err \tM_k x | \le 2\|\tM d\|_2 \|\cov_\err\|_{\op}\|x\|_2 \le 2\delta \|\tM d\|_2 \|x\|_2.$$

Since $\tM \preccurlyeq \sum_{k=0}^\kappa \Pi_k$, using \lref{lemma:chaining}, it follows that  $\|\tM d\|_2 \le \kappa \sqrt{\lambda^{-1} n \log(nT)}$ while $\|x\|_2 \le n$ because of \pref{prop:kls}. Then, by our choice of $\delta$, $$\lambda ~|d^\top \tM \cov_\err \tM_k x| \le \Phi^{-1}.$$

Plugging the above bounds in \eqref{eqn:lterm}, 
\begin{align}\label{eq:int1}
    \BE_{p(v)}[|L|\cdot\ind_{\CG}] &\ge  \frac{\lambda}{B} \cdot \frac34 \sum_{k=0}^\kappa 2^{-k} ~\BE_{w} [c_{k}(w)|\lambda  d^\top\tM_k w|] +  \frac{\lambda}{B} \cdot \frac14 \sum_{k=0}^\kappa  2^{-k} ~ \BE_{y} [c_{k}(y)|\lambda  d^\top\tM_k y|] - 4
\end{align}
where the second inequality follows since $\sum_{k=0}^\kappa \BE_x[|s_k(x)|] \le \Phi.$\\

To finish the proof, we use the inequality that $\cosh(a)a \ge \cosh(a) - 2$ for all $a \in \BR$ so that the first term is 
\begin{align*}
    \BE_{w} [c_{k}(w)|\lambda  d^\top\tM_k w|] ~\ge~ \BE_{w} [c_{k}(w)] - 2.
\end{align*}
\end{proof}







